Federated PCA on Grassmann Manifold for Anomaly Detection in IoT Networks

In the era of Internet of Things (IoT), network-wide anomaly detection is a crucial part of monitoring IoT networks due to the inherent security vulnerabilities of most IoT devices. Principal Components Analysis (PCA) has been proposed to separate network traffics into two disjoint subspaces corresponding to normal and malicious behaviors for anomaly detection. However, the privacy concerns and limitations of devices' computing resources compromise the practical effectiveness of PCA. We propose a federated PCA-based Grassmannian optimization framework that coordinates IoT devices to aggregate a joint profile of normal network behaviors for anomaly detection. First, we introduce a privacy-preserving federated PCA framework to simultaneously capture the profile of various IoT devices' traffic. Then, we investigate the alternating direction method of multipliers gradient-based learning on the Grassmann manifold to guarantee fast training and the absence of detecting latency using limited computational resources. Empirical results on the NSL-KDD dataset demonstrate that our method outperforms baseline approaches. Finally, we show that the Grassmann manifold algorithm is highly adapted for IoT anomaly detection, which permits drastically reducing the analysis time of the system. To the best of our knowledge, this is the first federated PCA algorithm for anomaly detection meeting the requirements of IoT networks.

==> experiment_setting.tex <==
\section{Description of the Dataset}

The KDDCup’99 dataset has been known as one of the most popular dataset for anomaly detection. This dataset has been developed based on the DARPA 98 dataset at the MIT Lincoln Laboratory, produced by the DARPA (1998) Intrusion Detection Evaluation Program. It included nine weeks of raw TCP dump data for a local area network (LAN) simulating a typical US Air Force LAN. The LAN was operated as if it were a true Air Force environment, but peppered with multiple attacks. Protocols such as TCP, UDP, and ICMP had been used on this dataset to evaluate the intrusion detection methods. The full KDDCup’99 dataset (uncompressed file kddcup.data.gz) has 4,898,431 records, and each record contains 41 features. Since the KDDCup’99 dataset contains so much data, many authors used a reduced version of the KDDCup’99 dataset (uncompressed file kddcup.data 10 percent.gz) to reduce the computation time. The kddcup.data 10 percent.gz is about 10\% of the KDDCup’99 dataset, and contains 494,021 records, of which 97,278 are normal (19.6\%) and 396,743 are intrusions (80.4\%). In the reduced version, the normal, neptune, smurf, ipsweep, nmap, portsweep, and satan instances are reduced. However, because even rare intrusion instances may severely compromise security, we used the full dataset for our experiments.



==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{sec.~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Sec.~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{secs. \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{Secs. \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{(\ref{#1})}
% Reference to an equation, upper case
\def\Eqref#1{(\ref{#1})}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{alg.~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Alg.~\ref{#1}}
\def\twoalgref#1#2{algs. \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algs. \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> math_content.tex <==
\section{Math Content}
To simplify notation, denote $\gF \defeq \ell \,\circ \, \gH \defeq \set{ z \mapsto \ell(z,h), h \in \gH }.$ 

We have
\begin{align}
	{\mathscr{L}(\widehat{P}_{\lambda}, f_{\theta}) :=
	\mathbf{E}_{Z \sim \widehat{P}_{\lambda}} \bigS{\ell(Z,  h_{\theta})}} \\
{\mathscr{L}({P}, f_{\theta}) \defeq \mathbf{E}_{Z \sim {P}} \bigS{\ell(Z,  h_{\theta})}}. \\
{\mathscr{L}({P}, f) \defeq \mathbf{E}_{Z \sim {P}} \bigS{\ell(Z,  h)}}.
\end{align}

\begin{align}
\mathscr{L}_{\rho}^{\gamma} (\widehat{P}_{\lambda},f) := & \mathbf{E}_{Z \sim \widehat{P}_{\lambda}}\Big{[}\phi_\gamma(Z, h)\Big{]} + \gamma \rho \\
\mathscr{L}_{\rho}^{\gamma} ({P},f) := & \mathbf{E}_{Z \sim {P}}\Big{[}\phi_\gamma(Z, h)\Big{]} + \gamma \rho. 
\end{align}

\textbf{Raginsky}: Suppose that $f$ is $L$-Lipschitz
\begin{align}
\mathscr{L}(Q, f) &\leq \mathscr{L}_{\rho}(P_{\lambda},f) \leq \mathscr{L}(Q,f) + 2L\rho, \;\forall Q \in \gB(P_{\lambda}, \rho) \\
\mathscr{L}(Q, f) &\leq \underset{S \in \gB({P}, \rho)}{\mbox{sup }} \mathscr{L} (S,f) \leq \mathscr{L}(Q,f) + 2L\rho, \;\forall Q \in \gB(P_{\lambda}, \rho)
\end{align}


\textbf{Proposition 1}: Suppose that $f$ is $L$-Lipschitz
\begin{align}
\mathscr{L}(Q,f) &\leq   \mathscr{L}_{\rho}^{\gamma}(P_{\lambda},f) \leq  \mathscr{L}(Q,f) + (2L + \gamma \mathbbm{1}_{\{\gamma \neq \gamma^{*}\}}) \, {\rho}, \;\forall Q \in \gB(P_{\lambda}, \rho) \\
%\mathscr{L}(Q,f) &\leq   \mathscr{L}(P_{\lambda},\phi_{\gamma}) \leq  \mathscr{L}(Q,f) + (2L + \gamma\mathbf{I}) \, {\rho}, \;\forall Q \in \gB(P_{\lambda}, \rho)
\end{align}

\begin{proof}
	The first inequality:
	\begin{align}
	\mathscr{L}(Q,f) \leq  \underset{S \in \gB({P}, \rho)}{\mbox{sup }} \mathscr{L} (S,f)  \leq  \mathscr{L}_{\rho}^{\gamma}(P_{\lambda},f) \\
%	\mathscr{L}(Q,f) \leq  \underset{S \in \gB({P}, \rho)}{\mbox{sup }} \mathscr{L} (S,f) \leq  \mathscr{L}(P_{\lambda},\phi_{\gamma})
	\end{align}
	
	The last "$ \leq $":
	
	\begin{align*} 
%	\mathscr{L}_{\rho}^{\gamma}(P_{\lambda},f)  & =  \mathscr{L}_{\rho}(P_{\lambda},f) + \mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, f)  - \mathscr{L}_{\rho}(P_{\lambda},f) \\
	\mathscr{L}_{\rho}^{\gamma}(P_{\lambda},f)   & =   \underset{S \in \gB({P}, \rho)}{\mbox{sup }} \mathscr{L} (S,f) + \mathscr{L}_{\rho}^{\gamma}(P_{\lambda},f)  - \underset{S \in \gB({P}, \rho)}{\mbox{sup }} \mathscr{L} (S,f) \\
	&\leq   \mathscr{L}(Q,f) + 2L\rho  + \mathbf{E}_{Z \sim P}[\phi_{\gamma}(Z, h)] + \rho\gamma - \min_{\gamma^{\prime} \geq 0} \Big\{ \rho \gamma^{\prime} + \mathbf{E}_{Z \sim P}[\phi_{\gamma'}(Z, h)] \Big\} \\
	& \leq   \mathscr{L}(Q,f) + 2L\rho + \max_{\gamma^{\prime} \geq 0}\bigg\{{\rho}(\gamma - \gamma^{\prime}) + \mathbf{E}_{Z \sim P}\Big[\phi_{\gamma}(Z, h) - \phi_{\gamma'}(Z, h)\Big]\bigg\} \\
	& =  \begin{aligned}[t] \mathscr{L}(Q,f) + 2L\rho + \max_{\gamma^{\prime} \geq 0}\Bigg\{\rho(\gamma - \gamma^{\prime}) + \mathbf{E}_{Z \sim P}\bigg[& \sup_{\zeta \in \mathcal{Z}} \Big\{ \ell(\zeta,h)  - \gamma d(\zeta,  Z) \Big\} \\ 
		& \quad - \sup_{\zeta \in \mathcal{Z}} \Big\{ \ell(\zeta,h) - \gamma^{\prime} d(\zeta,  Z)  \Big\} \bigg]\Bigg\} \end{aligned} \\
	& =  \mathscr{L}(Q,f) + 2L\rho + \max_{\gamma^{\prime} \geq 0}\Bigg\{\rho(\gamma - \gamma^{\prime}) + \mathbf{E}_{Z \sim P}\bigg[\sup_{\zeta \in \mathcal{Z}} \Big\{(\gamma^{\prime} - \gamma) d(\zeta,  Z)\Big\}\bigg]\Bigg\} \\
	& =  \mathscr{L}(Q,f) + 2L\rho + \underbrace{\max_{k \leq \gamma}\Bigg\{k\bigg(\rho - \mathbf{E}_{Z \sim P}\Big[\sup_{\zeta \in \mathcal{Z}} d(\zeta,  Z)\Big]\bigg)\Bigg\}}_{A} \\
	& \leq   \mathscr{L}(Q,f) + (2L + \gamma \, \mathbbm{1}_{\{\gamma \neq \gamma^{\prime}\}})\rho
	\end{align*}
	
	where $ k = \gamma - \gamma^{\prime} \Rightarrow \gamma^{\prime} = \gamma - k \geq 0 $
	because 
	\[
	A \leq \left\{\begin{array}{cc}{\gamma}{\rho} & \text { if } \rho \geq \mathbf{E}_{Z \sim P}\Big[\underset{\zeta \in \mathcal{Z}}{\sup}\big\{d(\zeta, Z)\big\}\Big]  \Rightarrow k=\gamma \\ 
	 \\ 0 & \text { if } \rho < ... \ k=0\end{array}\right.
	\]
	
\end{proof}

\begin{lemma} Suppose that $f'$ is $L_z$-Lipschitz
	 \[
	 	 \mathscr{L}(Q, f') - \inf_{f \in \mathcal{F}} \mathscr{L}(Q, f) \leq  \mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, f') - \inf_{f \in \mathcal{F}} \mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, f) + (2L + \gamma \mathbbm{1}_{\{\gamma \neq \gamma^{*}\}}) \rho, \; \forall Q \in \gB(P_{\lambda}, \rho). 
	 \]
	
\end{lemma}

\begin{proof}
	From proposition 1 and when $f_Q = \argmin_{f \in \mathcal{F}} \mathscr{L}(Q, f)$ is $L$-Lipschitz, we have:
	\begin{align}
		\mathscr{L}(Q, f') &\leq  \mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, f'),  \\ 
		\inf_{f \in \mathcal{F}} \mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, f) \leq  \mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, f_Q) &\leq \mathscr{L}(Q, f_{Q}) + (2 L+\gamma \mathbbm{1}_{\{\gamma \neq \gamma^{*}\}}) \rho \\
		&= \inf_{f \in \mathcal{F}} \mathscr{L}(Q, f) + (2 L+\gamma \mathbbm{1}_{\{\gamma \neq \gamma^{*}\}}) \rho. 
	\end{align}
	where  

\end{proof}

%\begin{theorem} If Assumption $\ell(Z,f)$ is $L_{\theta}$-Lipschitz continuous, then 
%	\[ 
%		\mathscr{L}(P_{\lambda}, \widehat{f}_{\theta^{\sigma}})- \inf_{f \in \mathcal{F}} \mathscr{L}(P_{\lambda}, f) \leq  \frac{\mathscr{C}(\gF)}{\sqrt{n}}+\epsilon + M \sqrt{\frac{2 \log (2 / \delta)}{n}} + (2L + \gamma) \hat{\rho}
%	\]
%	where:  
%	$\mathcal{F} = \bigC{f_{\theta}, \theta \in \Theta  \subset \mathbb{R}^d}$ and  $ \widehat{f}_{\theta^{\sigma}} \in \underset{\theta \in \Theta}{\operatorname{argmin}}\ \mathscr{L}(\widehat{P}_{\lambda}, f_{\theta}) + \sigma$, and 
%	$\mathscr{C}(\mathcal{F}):=\int_{0}^{\infty} \sqrt{\log \mathcal{N}\left(\mathcal{F},\|\cdot\|_{\infty}, \epsilon \right)} \mathrm{d} \epsilon$ and $\mathcal{N}\left(\mathcal{F},\|\cdot\|_{\infty}, \epsilon \right)$ denotes the covering number of $\mathcal{F}$ in the uniform metric $\ldots$.
%\end{theorem}

\begin{theorem} \label{Thrm:key} If Assumption $\ell(z,h_{\theta})$ is $L_{\theta}$-Lipschitz continuous, $\abs{\ell(z,h) } \leq M_{\ell}$ and considering the parametrized hypothesis class  $\mathcal{H} = \bigC{h_{\theta}, \theta \in \Theta  \subset \mathbb{R}^d}$, and $\forall Q \in \gB(P_{\lambda}, \rho)$, then 
	\[ 
	\mathscr{L}(Q, {f}_{\widehat{\theta}^{\varepsilon}})- \inf_{f \in \mathcal{F}} \mathscr{L}(Q, f) \leq  \sum_{i=1}^{m} \lambda_i \BiggS{\frac{48 \mathscr{C}(\Theta)}{\sqrt{n_i}} + 2 M_{\ell} \sqrt{\frac{2 \log (2  m / \delta)}{n_i}}} +\varepsilon + (2L + \gamma \mathbbm{1}_{\{\gamma \neq \gamma^{*}\}}) \rho
	\]
	with probability at least $1 - \delta$. Here $\widehat{\theta}^{\varepsilon}$ is the solution returned by FedRob after $O(1/\varepsilon)$ iterations, i.e., 
	  \begin{align}
	%  \mathscr{L}(\widehat{P}_{\lambda}, {f}_{\widehat{\theta}^{\varepsilon}}) &\defeq \mathbf{E}_{Z \sim \widehat{P}_{\lambda}} \bigS{\ell(Z,  h_{\widehat{\theta}^{\varepsilon}})}  \leq \underset{\theta \in \Theta} {\operatorname{inf}} \ \mathbf{E}_{Z \sim \widehat{P}_{\lambda}} \bigS{\ell(Z,  h_{\theta})}  + \varepsilon \\
	  \mathscr{L}_{\rho}^{\gamma} (\widehat{P}_{\lambda},f_{\widehat{\theta}^{\varepsilon}})  & \defeq \mathbf{E}_{Z \sim \widehat{P}_{\lambda}}\Big{[}\phi_\gamma(Z, h_{\widehat{\theta}^{\varepsilon}})\Big{]} + \gamma \rho \leq \underset{\theta \in \Theta} {\operatorname{inf}}  \BigS{\mathbf{E}_{Z \sim \widehat{P}_{\lambda}} \bigS{\phi(Z,  h_{\theta})}  + \gamma \rho } + \varepsilon
%	  {\widehat{\theta}^{\varepsilon}} \in \underset{\theta \in \Theta} {\operatorname{argmin}} \ \mathbf{E}_{Z \sim \widehat{P}_{\lambda}} \bigS{\ell(Z,  h_{\theta})}  + \varepsilon
	  \end{align}
	  and 
	$\mathscr{C}(\Theta):= L_{\theta} \int_{0}^{\infty} \sqrt{\log \mathcal{N}\left(\Theta,\|\cdot\|_{\Theta}, \epsilon \right)} \mathrm{d} \epsilon$ where $\mathcal{N}\left(\Theta,\|\cdot\|_{\Theta}, \epsilon \right)$ denotes the $\epsilon$-covering number of $\Theta$ w.r.t  a  metric $\|\cdot\|_{\Theta}$ as the norm on $\Theta$.
\end{theorem}

\textbf{Remarks:}
Choose $\varepsilon$ in the order of $1/\sqrt{n}$. 

\begin{proof}
	To simplify notation, we denote $ \Phi \defeq \phi_{\gamma} \circ \mathcal{H} = \set{z \mapsto \phi_{\gamma}(z, h), h \in \mathcal{H}}$ where $\mathcal{H} = \bigC{h_{\theta}, \theta \in \Theta  \subset \mathbb{R}^d}$, which represents the composition of $\phi_{\gamma}$ with each of the predictor function $h_{\theta}$ parametrized by $\theta$ belonging to a parameter class $\Theta$. 
	
	Defining $f_P \in \argmin_{f \in \mathcal{F}} \mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, f)$ and $ \widehat{\theta}^* \in \underset{\theta \in \Theta} {\operatorname{argmin}} \ \mathbf{E}_{Z \sim \widehat{P}_{\lambda}} \bigS{\phi(Z,  h_{\theta})}$ such that $\mathscr{L}_{\rho}^{\gamma}(\widehat{P}_{\lambda}, {f}_{\widehat{\theta}^*}) = \underset{\theta \in \Theta} {\operatorname{inf}}  \BigS{\mathbf{E}_{Z \sim \widehat{P}_{\lambda}} \bigS{\phi(Z,  h_{\theta})}  + \gamma \rho }$, we  decompose the excess risk as follows:
	
	\begin{align}
	&\mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, {f}_{\widehat{\theta}^{\varepsilon}}) - \inf_{f \in \mathcal{F}}  \mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, f) \nonumber\\
	&= \mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, {f}_{\widehat{\theta}^{\varepsilon}}) -   \mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, f_P)\nonumber\\
	&=  \BigS{\mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, {f}_{\widehat{\theta}^{\varepsilon}}) - \mathscr{L}_{\rho}^{\gamma}(\widehat{P}_{\lambda}, {f}_{\widehat{\theta}^{\varepsilon}})} + \underbrace{\BigS{\mathscr{L}_{\rho}^{\gamma}(\widehat{P}_{\lambda}, {f}_{\widehat{\theta}^{\varepsilon}}) - \mathscr{L}_{\rho}^{\gamma}(\widehat{P}_{\lambda}, {f}_{\widehat{\theta}^{*}})} }_{\leq \varepsilon} + \underbrace{\BigS{\mathscr{L}_{\rho}^{\gamma}(\widehat{P}_{\lambda}, {f}_{\widehat{\theta}^{*}}) - \mathscr{L}_{\rho}^{\gamma}(\widehat{P}_{\lambda}, f_P)}}_{\leq 0} \nonumber\\
	& \quad  + \BigS{\mathscr{L}_{\rho}^{\gamma}(\widehat{P}_{\lambda}, f_P) - \mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, f_P)} \nonumber\\
%	& \leq 2 \sup_{f \in \mathcal{F}} \; \big\lvert\mathscr{L}_{\rho}^{\gamma}(P_{\lambda}, f) - \mathscr{L}_{\rho}^{\gamma}(\widehat{P}_{\lambda}, f) \big\rvert  + \varepsilon\\
	&\leq 2 \sup_{\phi_{\gamma} \in \Phi} \abs*{ \mathbf{E}_{Z \sim P_{\lambda}}[\phi_{\gamma}(Z, h_{\theta})] -   \mathbf{E}_{Z \sim \widehat{P}_{\lambda}}[\phi_{\gamma}(Z, h_{\theta})] } + \varepsilon \nonumber\\
	&\leq 2 \sup_{\phi_{\gamma} \in \Phi}  \sum_{i=1}^{m} \lambda_i \abs*{\mathbf{E}_{Z_i \sim P_i}[\phi_{\gamma}(Z_i, h_{\theta})] -   \mathbf{E}_{Z_i \sim \widehat{P}_{i}}[\phi_{\gamma}(Z_i, h_{\theta})]}  + \varepsilon \nonumber\\
	&\leq 2   \sum_{i=1}^{m} \lambda_i \sup_{\phi_{\gamma} \in \Phi} \abs*{\mathbf{E}_{Z_i \sim P_i}[\phi_{\gamma}(Z_i, h_{\theta})] -   \mathbf{E}_{Z_i \sim \widehat{P}_{i}}[\phi_{\gamma}(Z_i, h_{\theta})]}  + \varepsilon \nonumber\\
	%&\stackrel{\text {with prob. } \geq 1-\delta}{\leq}  
	& \leq  \sum_{i=1}^{m} \lambda_i  \biggS{4 \mathscr{R}_{i}(\Phi)+  2 M_{\ell} \sqrt{\frac{2 \log (2 m / \delta)}{n_i}}} + \varepsilon\, \text{  with probability at least }  1-\delta, \label{unionbound1}
	\end{align}
where the first inequality is due to optimization error and definition of $\widehat{\theta}^{*}$. The second inequality is due to the fact that $ \abs{\sum_{i=1}^m \lambda_i a_i } \leq \sum_{i=1}^m \lambda_i  \abs{a_i}, \forall a_i \in \mathbb{R}$ and $\lambda_i \geq 0$. The third inequality is because pushing the $\sup$ inside increases the value. For the last inequality, using  the facts that (i) $\abs{\phi_{\gamma}(z,h)} \leq M_{\ell}$  due to $-M_{\ell} \leq \ell(z, h) \leq \phi_{\gamma}(z, h) \leq \sup _{z \in \gZ} \ell(z, h) \leq M_{\ell}$ and (ii) the Rademacher complexity of the function class $\Phi$ defined by $\mathscr{R}_{i}(\Phi) = \mathbf{E}[\sup _{\phi_{\gamma} \in \Phi} \frac{1}{n_i} \sum_{k=1}^{n_i} \sigma_{k} \phi_\gamma(Z_k,  h_{\theta})] $ where the expectation is w.r.t both $Z_k \stackrel{\text { i.i.d. }}{\sim} P_i$ and i.i.d. Rademacher random variable $\sigma_{k}$ independent of $Z_k, \forall k \in [n_i]$,  we have 
\begin{align}
\sup_{\phi_{\gamma} \in \Phi} \abs*{\mathbf{E}_{Z_i \sim P_i}[\phi_{\gamma}(Z_i, h_{\theta})] -   \mathbf{E}_{Z_i \sim \widehat{P}_{i}}[\phi_{\gamma}(Z_i, h_{\theta})]}  \geq 2 \mathscr{R}_{i}(\Phi)+   M_{\ell} \sqrt{\frac{2 \log (2 m / \delta)}{n_i}} \label{Rade1}
\end{align}
with probability $\leq \delta/m$ due to the standard symmetrization argument and McDiarmid's inequality \blue{[UnderstandingML, Theorem26.5]}. Multiplying $\lambda_i$ to both sides of \eqref{Rade1}, summing up the inequalities over all $i\in [n]$, and using union bound, we obtain \eqref{unionbound1}.


%Conditioning on the vector $Z_1^n \defeq (Z_k)_{k\in [n]}$, the above expectation gives us the empirical Rademacher complexity denoted by $\widehat{\mathscr{R}}_{n}(\Phi)$. 
Define a stochastic process $\left(X_{\phi_{\gamma}}\right)_{\phi_{\gamma} \in \Phi}$ 
$$
X_{\phi_{\gamma}}:=\frac{1}{{\sqrt{n_i}}} \sum_{k=1}^{n_i} \sigma_{k} \phi_{\gamma}(Z_k, h_{\theta})
$$
which is  zero-mean because $\mathbf{E}\left[X_{\phi_{\gamma}}\right]=0$ for all $\phi_{\gamma} \in \Phi$.  To upper-bound  $\mathscr{R}_{n}(\Phi)$, we first show that $\left(X_{\phi_{\gamma}}\right)_{\phi_{\gamma} \in \Phi}$ is a sub-Gaussian process with respect to the following pseudometric
\begin{align}
%\left\|\phi_{\gamma}-\phi_{\gamma}^{\prime}\right\|_{L_2(\widehat{P}_{\lambda})}  \defeq \biggP{\frac{1}{n} \sum_{k=1}^{n}  \BigP{\phi_{\gamma}(Z_k, f_{\theta}) - \phi_{\gamma}(Z_k, h_{\theta'})}^2}^{1/2}. 
\left\|\phi_{\gamma}-\phi_{\gamma}^{\prime}\right\|_{\infty}  \defeq  \sup_{z \in \mathcal{Z}} \Big\lvert  {\phi_{\gamma}(z, h_{\theta}) - \phi_{\gamma}(z, h_{\theta'})}  \Big\rvert . 
\end{align}  

For any $t \in \mathbb{R}$,  using Hoeffding inequality with the fact that $\sigma_{k}, k \in [n]$, are i.i.d. bounded random variable with sub-Gaussian  parameter 1, we have
$$
\begin{aligned}
\mathbf{E}\left[\exp \left(t\left(X_{\phi_{\gamma}}-X_{\phi_{\gamma}^{\prime}}\right)\right)\right] &=\mathbf{E}\left[\exp \left(\frac{t}{\sqrt{n_i}} \sum_{k=1}^{n_i} \sigma_{k}\left(\phi_{\gamma}\left(Z_k, h_{\theta}\right)-\phi\left(Z_k, h_{\theta'}\right)\right)\right)\right] \\
&=\left(\mathbf{E}\left[\exp \left(\frac{t}{{\sqrt{n_i}}} \sigma_{1}\left(\phi_{\gamma}\left(Z_{1}, h_{\theta}\right)-\phi_{\gamma}\left(Z_{1}, h_{\theta'}\right)\right)\right)\right]\right)^{n_i} \\
%& \leq \exp \left(\frac{t^{2} \left\|\phi_{\gamma}-\phi_{\gamma}^{\prime}\right\|_{L_2(\widehat{P}_{\lambda})}^{2}}{2 }\right). 
& \leq \exp \left(\frac{t^{2} \left\|\phi_{\gamma}-\phi_{\gamma}^{\prime}\right\|_{\infty}^2}{2 }\right). 
\end{aligned}
$$
Then, invoking Dudley entropy integral, we have
\begin{align}
\sqrt{n_i}\, {\mathscr{R}}_{i}(\Phi) = \mathbf{E} \sup_{\phi_{\gamma} \in \Phi} X_{\phi_{\gamma}} \leq {12} \int_{0}^{\infty} \sqrt{\log \mathcal{N}\left(\Phi, \norm{\cdot}_{\infty}, \epsilon\right)} \mathrm{d} \epsilon
\end{align}

We will show that when $\theta \mapsto \ell(z,h_{\theta})$ is $L_{\theta}$-Lipschitz, then $\theta \mapsto \phi_{\gamma}(z, h_{\theta})$ is also $L_{\theta}$-Lipschitz. First, we have
\begin{align*}
	\Big|\phi_{\gamma}(z, h_{\theta}) - \phi_{\gamma}(z, h_{\theta'})\Big|  &=  \bigg| \sup_{\zeta \in \mathcal{Z}} \inf_{\zeta' \in \mathcal{Z}} \Big\{ \ell(\zeta,h_{\theta})  - \gamma d(\zeta,  z)   -   \ell(\zeta', h_{\theta'}) + \gamma d(\zeta',  z)  \Big\} \bigg| \\
	&\leq  \bigg| \sup_{\zeta \in \mathcal{Z}} \Big\{ \ell(\zeta,h_{\theta})    -   \ell(\zeta, h_{\theta'})   \Big\} \bigg| \\
	&\leq \sup_{\zeta \in \mathcal{Z}}  \bigg| \Big\{ \ell(\zeta,h_{\theta})    -   \ell(\zeta, h_{\theta'})   \Big\} \bigg| \\
	& \leq L_{\theta}   \norm{\theta - \theta'}, \\
	%& \leq L_f L_{\theta} \norm{\theta - \theta'}
\end{align*}
which implies
\begin{align}
\left\|\phi_{\gamma}-\phi_{\gamma}^{\prime}\right\|_{\infty} \leq  L_{\theta}   \norm{\theta - \theta'}.
\end{align}
Therefore, by contraction principle \blue{[Understanding ML]}, we have
\begin{align}
\mathcal{N}\left(\Phi, \norm{\cdot}_{\infty}, \epsilon\right) \leq \mathcal{N}\left(\Theta, \norm{\cdot}, \epsilon/L_{\theta}\right)
\end{align}
\end{proof}

\begin{proposition}[Measure concentration (Fournier and Guillin, 2015, Theorem 2)]\label{WassRate}
	Let $P$ be a probability distribution on a bounded set $\mathcal{Z}$. Let $\widehat{P}_{n}$ denote the empirical distribution of $Z_{1}, \ldots, Z_{n} \stackrel{\text { i.i.d. }}{\sim} P.$ Assuming that there exist constants $a>1$  such that $A \defeq \mathbf{E}_{Z \sim P}\bigS{\exp(\norm{Z}^a)} < \infty$ (i.e., $P$ is a light-tail distribution). Then, for any $\rho > 0$,
$$
%\mathbf{P}\left[ W (P_{\lambda}, \widehat{P}_{n}) \geq  \rho \right] \leq c_{1} \exp \left(-c_{2} n \rho^{\max\{d+1, 2\}}\right) \\
\mathbf{P}\left[ W (\widehat{P}_{n}, P) \geq  \rho \right]  \leq \begin{cases}c_{1} \exp \left(-c_{2} n \rho^{\max \{d+1,2\}}\right) & \text { if } \rho \leq 1 \\ c_{1} \exp \left(-c_{2} n \rho^{a}\right) & \text { if } \rho>1\end{cases}
$$
where $c_{1}, c_{2}$ are constants depending on $a, A$ and $d$.
\end{proposition}
As a consequence of this proposition,  for any $\delta > 0$, we have  
\begin{align}\label{E:deltarho}
\mathbf{P}\left[ W (\widehat{P}_{n}, P) \leq  \widehat{\rho}_{n}^{\delta} \right] \geq 1 - \delta \; \text{  where  } \; \widehat{\rho}_{n}^{\delta} \defeq \begin{cases}\left(\frac{\log \left(c_{1} / \delta \right)}{c_{2} n}\right)^{\min \{1 / (d+1), 1 / 2\}} & \text { if } n \geq \frac{\log \left(c_{1} / \delta\right)}{c_{2}}, \\ \left(\frac{\log \left(c_{1} / \delta\right)}{c_{2} n}\right)^{1 / \alpha} & \text { if } n<\frac{\log \left(c_{1} / \delta\right)}{c_{2}}.\end{cases}
\end{align}

\begin{corollary}
	With all assumptions as in Theorem~, we have
	\[ 
	\mathscr{L}(P_{\lambda}, {f}_{\widehat{\theta}^{\varepsilon}})- \inf_{f \in \mathcal{F}} \mathscr{L}(P_{\lambda}, f) \leq  \sum_{i=1}^{m} \lambda_i \BiggS{\frac{48 \mathscr{C}(\Theta)}{\sqrt{n_i}} + 2 M_{\ell} \sqrt{\frac{2 \log (4  m / \delta)}{n_i}} + \bigP{2L + \gamma \mathbbm{1}_{\{\gamma \neq \gamma^{*}\}} }\widehat{\rho}_{n_i}^{\delta/2m} } +\varepsilon
	\]
	with probability at least $1 - \delta$. 
\end{corollary}
\begin{proof}
We will exploit the joint convexity property of 1-Wasserstein distance, which can be shown as the mapping $(\alpha, \beta) \mapsto W(\alpha, \beta)$ is convex. To see that, by Kantorovich-Rubinstein Duality,  we have $W(\alpha, \beta) = \sup_{\norm{f}_L \leq 1} \mathbf{E}_{\alpha}[f] - \mathbf{E}_{\beta}[f] =  \sup_{\norm{f}_L \leq 1} T_f (\alpha, \beta)$, which is the sumpremum of linear functions $T_f: \gP \times \gP \mapsto \mathbb{R}$ defined by $T_f (\alpha, \beta) = (\alpha, \beta)^{\top}(f, -f)$, and thus the convexity follows. Thus we have 
\begin{align}
W(P_{\lambda}, \widehat{P}_{\lambda}) = W \BigP{\sum\limits_{i=1}^m \lambda_i (\widehat{P}_i, P_i)} \leq  {\sum\limits_{i=1}^m \lambda_i W(\widehat{P}_i, P_i)}.
\end{align}
Then, we have
\begin{align}
\mathbf{P}\BigS{W(P_{\lambda}, \widehat{P}_{\lambda}) \geq \sum\limits_{i=1}^{m} \lambda_i \widehat{\rho}_{n_i}^{\delta/2m} }
&\leq \mathbf{P}\BigS{\sum\limits_{i=1}^m \lambda_i W(\widehat{P}_i, P_i) \geq \sum\limits_{i=1}^{m} \lambda_i \widehat{\rho}_{n_i}^{\delta/2m} } \nonumber\\
&\leq \sum\limits_{i=1}^m  \mathbf{P}\BigS{ W(\widehat{P}_i, P_i) \geq   \widehat{\rho}_{n_i}^{\delta/2m} } \nonumber\\
&\leq \sum\limits_{i=1}^m  \frac{\delta}{2 m}= \frac{\delta}{2}, \label{E:barry}
\end{align}
where the second inequality is due to the union bound, and the third inequality is due to  Proposition~\ref{WassRate} and \eqref{E:deltarho}. By setting $\rho = \sum\limits_{i=1}^{m} \lambda_i \widehat{\rho}_{n_i}^{\delta/2m}$  in Theorem~\ref{Thrm:key} and using union bound, we complete the proof. 
\end{proof}

\subsection{How to choose $\lambda$}
Controlling $\lambda$ for various purpose: either adapt to a specific domain or covering all clients with minimum $\rho$. 

For domain adaptation
\begin{align}
\min_{\lambda \in \Delta} W(\widehat{P}_{\lambda}, \widehat{Q}) \leq \min_{\lambda \in \Delta} \sum\limits_{i=1}^{m} \lambda_i W(\widehat{P}_i, \widehat{Q}) 
\end{align}

For covering all client distribution, based on the Wasserstein barycenter problem
\begin{align}
W(\widehat{P}_{{\lambda}^*}, {P}^*) \leq  \min_{\lambda \in \Delta, Q \in \gP} \sum\limits_{i=1}^{m} \lambda_i W(\widehat{P}_i, {Q}) \defeq \rho^*
\end{align}

By triangle inequality:
\begin{align}
W(P_{\lambda^*}, P_j) &\leq W(P_{\lambda^*}, \widehat{P}_{\lambda^*}) + W(\widehat{P}_{\lambda^*}, P^*) + W( P^*, \widehat{P}_j) + W(  \widehat{P}_j, P_j) \nonumber\\
& \leq \sum\limits_{i=1}^{m} \lambda_i^* \widehat{\rho}_{n_i}^{\delta/2m} + \rho^* + \frac{\rho^*}{\lambda_j} + \widehat{\rho}_{n_j}^{\delta/2} \; \text{  with probability at least }  1-\delta, \label{E:bary2}
\end{align}
where \eqref{E:bary2} is due to several facts: (i) $\mathbf{P}\bigS{W(P_{\lambda^*}, \widehat{P}_{\lambda^*}) \geq \sum\limits_{i=1}^{m} \lambda_i^* \widehat{\rho}_{n_i}^{\delta/2m} } \leq \delta/2$ according to \eqref{E:barry}, (ii) $W( P^*, \widehat{P}_j) = \frac{\lambda_j W( P^*, \widehat{P}_j)}{\lambda_j}\leq \frac{\rho^*}{\lambda_j}$, and (iii)  $\mathbf{P}\bigS{W(  \widehat{P}_j, P_j) \geq \widehat{\rho}_{n_j}^{\delta/2} } \leq \delta/2$ according to \eqref{E:deltarho}, and (iv) using union bound. 

\begin{lemma}
\begin{align*}
	\mathscr{L}_{\rho}^{\gamma}(Q, f) & = \mathscr{L}_{\rho}^{\gamma}(Q,f) + \mathscr{L}_{\rho_{\gamma}}^{\gamma}(Q,f) - \mathscr{L}_{\rho}^{\gamma}(Q,f) \\		
	& = \mathscr{L}_{\rho}^{\gamma}(Q, f)+\gamma(\rho - f_{\gamma}) \\
	& \leq  \mathscr{L}(Q, f) + (2L + \gamma\mathbf{I}_{\{\gamma \neq \gamma^{\prime}\}})\rho		
\end{align*}
\end{lemma}

\textbf{Tuning}:
\begin{enumerate}
	\item Choose the desire $\rho^{*}$
	\item Adjust $\gamma$ to have $\rho_{\gamma} = \rho^{*}$
\end{enumerate}


